Optimizing Contextual Speech Recognition Using Vector Quantization for Efficient Retrieval

Neural contextual biasing allows speech recognition models to leverage contextually relevant information, leading to improved transcription accuracy. However, the biasing mechanism is typically based on a cross-attention module between the audio and a catalogue of biasing entries, which means computational complexity can pose severe practical limitations on the size of the biasing catalogue and consequently on accuracy improvements. This work proposes an approximation to cross-attention scoring based on vector quantization and enables compute- and memory-efficient use of large biasing catalogues. We propose to use this technique jointly with a retrieval based contextual biasing approach. First, we use an efficient quantized retrieval module to shortlist biasing entries by grounding them on audio. Then we use retrieved entries for biasing. Since the proposed approach is agnostic to the biasing method, we investigate using full cross-attention, LLM prompting, and a combination of the two. We show that retrieval based shortlisting allows the system to efficiently leverage biasing catalogues of several thousands of entries, resulting in up to 71% relative error rate reduction in personal entity recognition. At the same time, the proposed approximation algorithm reduces compute time by 20% and memory usage by 85-95%, for lists of up to one million entries, when compared to standard dot-product cross-attention.

==> intro_OLD.tex <==
\section{Introduction}
\label{sect:intro}

\IEEEPARstart{E}{nd-to-end} deep learning models have revolutionized the field of automatic speech recognition (ASR) during the last few years, offering both simplicity and impressive performance~\cite{prabhavalkar2023end}. However, even large models trained on vast amounts of data can still struggle with recognizing words that are rare or even unseen during training---a scenario especially common in case of entities such as personal or geo-location names~\cite{guo2019spelling, sainath2018no, alon2019contextual}. One way to address this problem is to allow models to use user-specific information, or context, during inference. Such context is often referred to as the user's biasing catalogue, and can include contact names, commonly used apps, media titles and creators, or relevant geo-locations. %names. 

To that end, several approaches have been proposed in the literature, including shallow language model (LM) fusion~\cite{zhao2019shallow, le2021deep} and on-the-fly LM-based rescoring~\cite{hall2015composition, williams2018contextual}. Such methods, though, are often sub-optimal, because of the well-documented tendency of end-to-end models to learn a strong internal LM~\cite{mcdermott2021dr, meng2021internal}, and because the contextual model is trained independently from the acoustic model (AM). Neural contextual biasing (NCB) offers an alternative paradigm wherein the biasing machinery is part of the ASR model and is jointly learnt with the main ASR objective~\cite{pundak2018deep, chang2021context, sathyendra2022contextual, bruguier2019phoebe, jain2020contextual, sun2021tree, munkhdalai2022fast, meng2024text}. 

NCB architectures usually rely on an additional context encoder followed by a fusion mechanism. The context encoder may be implemented as an LSTM~\cite{hochreiter1997long}, or more recently a transformer~\cite{vaswani2017attention} module, and its role is to map a set of tokenized biasing phrases to a set of fixed-length continuous embeddings. Next, these embeddings are integrated with the acoustic 
%(in case of transducer~\cite{graves2012sequence} or attention encoder-decoder (AED) ASR architectures~\cite{chan2015listen}) and/or label (in case of transducer ASR architectures) 
encoder when making ASR predictions, with the integration typically taking place in a latent space with cross-attention between the audio  
and context encoders~\cite{pundak2018deep, jain2020contextual}.
%at the output of the audio encoder, though some recent works report improved performance by doing fusion via one or more intermediate audio encoder layers~\cite{peng-etal-2024-owsm,huang2024contextual,Torres2024promptformer}.

Another approach relies on utilizing large language models (LLMs) for contextualization. LLMs are transformer-based models with billions of parameters that have yielded exciting results in general-purpose natural language understanding and generation~\cite{minaee2024large}. The speech community has been exploring ways to incorpotate the power of LLMs into ASR decoding~\cite{rubenstein2023audiopalm,seide2024speech,yang2024promptasr,lakomkin2024end,chen2024its}, with shallow fusion~\cite{hu2023massively}, n-best rescoring~\cite{xu2022rescorebert}, and error correction re-decoding~\cite{yang2023generative} being some of the proposed approaches. Delayed fusion (DF) has been also recently introduced as a promising alternative~\cite{hori2025_df}, allowing to use already trained---potentially with very different vocabularies---ASR and LLM models, without the need of acquiring long (and computationally demanding) n-bset lists. LLM reasoning can be further improved by injecting query-specific information via prompts~\cite{minaee2024large}, a property that has drawn particular attention for contextual biasing~\cite{gong2024contextual,Wang2023_slm,chen2024salm,lei2024contextualization}.

%\PAWEL{Write about using prompting contextualziation here, then explain the prompt capacity issue. Which is a nice detour into memory issue, retrieval, etc.} 

%Fusion can be implemented in a latent space with cross-attention between audio and context encoders~\cite{pundak2018deep, jain2020contextual} or by interpolating generic and contextual model's distributions, as done in tree-constrained pointer generation networks (TCPGN)~\cite{sun2021tree}. 
%Deep contextual biasing has been proposed for the CLAS~\cite{pundak2018deep, chan2015listen} AED model, and similar solutions were extended to the contextual neural transducers~\cite{graves2012sequence, jain2020contextual, chang2021context}. 

However, the described biasing machinery, based either on LLM prompting or on cross-attention fusion, comes at the cost of increased compute and memory, as well as potential accuracy degradation as the biasing inventory gets larger~\cite{Alexandridis2023,yang23o_interspeech,pundak2018deep,gong2024contextual}. On the one hand, LLMs have a specific maximum context length, typically in the range of a few thousand tokens~\cite{minaee2024large}. Even without reaching their technical full capacity, attention-based LLMs can be very inefficient for long contexts~\cite{minaee2024large}, and it has been reported that their accuracy can quickly get sub-optimal~\cite{levy-etal-2024-task}. On the other hand, cross-attention, generally implemented as scaled dot-product~\cite{vaswani2017attention}, needs to be applied between all the contextual embeddings (keys) and all the acoustic encodings (queries), something that can increase the time and space complexity to prohibitive levels as the length of the biasing list grows. 

Of course, attention is a ubiquitous technology across the machine learning community~\cite{niu2021review}, and significant effort has been focused on developing efficient implementations. For instance, flash attention~\cite{dao2022flashattention} introduces substantial speed gains by optimizing the read and write operations between different levels of memory, while ring attention~\cite{liu2023ring} offers an elegant way to parallelize the attention computation across multiple devices following block-wise processing. Such approaches, though, are hardware-oriented and do not provide algorithmically efficient solutions to decrease the overall compute and memory budget, especially on edge devices where due to privacy benefits much of the personalization aspect usually takes place. 
\IEEEpubidadjcol

In an effort to improve the computational efficiency of the biasing mechanism, some works have proposed to constrain NCB to be only triggered on a subset of relevant audio frames, something that also helps with the phenomenon of over-biasing~\cite{tong2023slot, Alexandridis2023}. Such approaches, despite limiting the number of time steps for which the dot-products need to be estimated, still do not offer a scalable solution with respect to the length of the biasing list. Those scalability limitations have led the research community to typically explore NCB settings where the biasing inventories are capped to a few thousand phrases at most \cite{pundak2018deep,tong2023slot,chen2019joint,Kulshreshtha2023,sudo2024contextualized}. To address the issue, other works dynamically limit the number of relevant phrases throughout decoding based on prefixes that appear in the partial hypotheses, applying bias-conditioning~\cite{pundak2018deep} or representing the biasing lists with prefix-trees~\cite{le2021deep,le21_interspeech,sun2021tree}. However, those techniques need access to the decoding history and are not flexible enough to be applied to non auto-regressive (e.g., CTC-based~\cite{graves2006}) models.

One way to potentially allow for a larger initial inventory in a flexible manner is to follow a two-stage, retrieval-based approach. In that line of work, the authors in~\cite{han2022improving,Munkhdalai2023nam,wu2024context,meng2024text} apply a phrase-level attention at the first pass to select a few candidate biasing phrases before applying a more expensive wordpiece-level attention in the second pass~\cite{munkhdalai2022fast}. 
%This idea is extended in~\cite{wu2024context}, where the computational complexity of the first pass is further reduced by employing a smaller contextual encoder, as well. 
However, this approach tries to deal with the \emph{additional} latency introduced by the wordpieces, thus still struggling to scale well with the number of biasing entries. A two-stage method is also introduced in~\cite{yang23o_interspeech}, where the phone sequence of the streaming ASR output is used to filter out irrelevant entries of the biasing list, according to certain confidence criteria. The phonemic information is also used in~\cite{lei2024contextualization}, where a few candidate entities from a first decoding pass guide an LLM-based retrieval of phonologically close entries that prompt the LLM during a second-pass decoding. Another closely related work is dual attention~\cite{Fu2019dual_attention}, a technique recently applied to the keyword spotting problem~\cite{sahai2023dual}. The idea relies on having two attention modules, a small and a large (full) one, and to conditionally execute either of them depending on some triggering signals. 

Retrieval approaches for ASR contextualization often operate in the linguistic~\cite{Bolaji2023_retr} or acoustic embedding space~\cite{wang2023_s2t_retrieval, Wang2023_slm}, where the embeddings then act as queries to retrieve k nearest neighbours (kNN)~\cite{Bolaji2023_retr} from a pre-built entity index, optionally using an auxiliary retrieval model~\cite{wang2023_s2t_retrieval, huang2024_retr}. Recently, a joint approach has been explored, where the retrieval step is part of the contextual ASR model~\cite{wu2024context,huang2024_retr}; in this case some form of dot-product score is still used to shortlist biasing entries, potentially with additional retrieval oriented loss. The kNN and attention approaches are compared in~\cite{gourav2024multi}, for the case of multi-modal LLMs.

In this work we address the attention-driven computational limitations of NCB employing a quantization-based, two-stage module, without the need for phonemic information, or other confidence signals. In more detail, we discretize the contextual embeddings using finite scalar quantization (FSQ), a variant of vector quantization~\cite{vq_2017} recently introduced in generative machine learning architectures~\cite{fsq_2024}. Utilizing certain properties of FSQ, we are able to approximate cross-attention in a memory- and runtime-efficient way, and use this efficient implementation to accurately retrieve a few relevant biasing entries. This subset of contextual phrases is then either (i)~integrated with the acoustic encodings through a full cross-attention biasing mechanism, or (ii)~used for LLM prompting in a delayed fusion manner.  

The main contributions of this paper are thus as follows: 
\begin{enumerate}
    \item We introduce vector quantization in the field of contextual speech recognition as a viable way to discretize the biasing embeddings and approximate the compute-heavy cross-attention mechanism, achieving over 20\% speed boost and 85-95\% memory usage reduction when the biasing list is large.
    \item We use our proposed approach in a retrieval mode, allowing us to efficiently shortlist phrases from large biasing catalogues. We show that the proposed approach can offer up to 71\% relative error rate reduction for entity recognition when compared to non-biased baselines.
    \item We pair our retrieval approach with different biasing implementations (full cross-attention, LLM prompting) and decoding configurations (in auto-regressive or non auto-regressive mode), demonstrating that our approach is flexible and agnostic to the exact biasing mechanism and decoding algorithm.
    \item Our work opens up a way to scale neural contextualization to relatively unexplored scenarios such as the media domain, where the number of entries could be in the hundreds of thousands or even millions.
\end{enumerate}

%The remainder of the paper is organized as follows: Section~\ref{sect:ncb} gives an overview of the cross-attention-based NCB as we use it in this work; in Sections~\ref{sect:vq} and~\ref{sect:vq_algo} we describe vector quantization and provide an in-depth analysis of the proposed algorithm we use to approximate cross-attention through FSQ; in Section~\ref{sect:expt} we showcase the effectiveness of our algorithm through experimental results on a large entity-rich dataset, scaling the length of the biasing list up to 43k entries; we conclude the paper discussing limitations and opportunities for future research in Section~\ref{sect:conclusions}.
